Factorized Quadruples and a Predictor of Higher-Level Correlation in Thermochemistry

Coupled cluster theory has had a momentous impact on the ab initio prediction of molecular properties, and remains a staple ingratiate in high-accuracy thermochemical model chemistries. However, these methods require inclusion of at least some connected quadruple excitations, which generally scale at best as $\mathcal{O}(N^9)$ with the number of basis functions. It very difficult to predict, a priori, the effect correlation past CCSD(T) has on a give reaction energies. The purpose of this work is to examine cost-effective quadruple corrections based on the factorization theorem of many-body perturbation theory that may address these challenges. We show that the $\mathcal{O}(N^7)$, factorized CCSD(TQ${}_\text{f}$) method introduces minimal error to predicted correlation and reaction energies as compared to the $\mathcal{O}(N^9)$ CCSD(TQ). Further, we examine the performance of Goodson's continued fraction method in the estimation of CCSDT(Q)${}_\Lambda$ contributions to reaction energies, as well as a "new" method related to %TAE[(T)] that we refer to as a scaled perturbation estimator. We find that the scaled perturbation estimator based upon CCSD(TQ${}_\text{f}$)/cc-pVDZ is capable of predicting CCSDT(Q)${}_\Lambda$/cc-pVDZ contributions to reaction energies with an average error of 0.07 kcal mol${}^{-1}$ and a RMST of 0.52 kcal mol${}^{-1}$ when applied to a test-suite of nearly 3000 reactions. This offers a means by which to reliably ballpark how important post-CCSD(T) contributions are to reaction energies while incurring no more than CCSD(T) formal cost and a little mental math.

==> src/abstract.tex <==
Since its inception, coupled cluster theory has had a momentous impact on the \textit{ab initio} prediction of molecular properties. In many cases, highly accurate results are obtainable within a computationally efficient, albeit high-order polynomial algorithm. If high-accuracy results are needed, as is frequently the case  for \textit{in silico} predictive thermochemistry, at least partial inclusion of connected quadruple excitations are required, which generally scale at best as $\mathcal{O}(N^9)$ with the number of basis functions. Frustratingly, it is rarely straightforward to ascertain the relative magnitude that electron correlation past CCSD(T) has on reaction energies a priori, though methods such as Goodson's continued fraction approximation and Martin's \%TAE[(T)] have seen some use in this regard. The purpose of this work is to determine the utility of cost-effective quadruple corrections based on the factorization theorem of many-body perturbation theory; both in terms of a potential tool in thermochemistry as well as an indicator for when a description of higher-rank excitations become important.  We show that the $\mathcal{O}(N^7)$, factorized CCSD(T\Qf{}) method introduces minimal error to predicted correlation and reaction energies as compared to the $\mathcal{O}(N^9)$ CCSD(TQ). Furthermore, we examine the performance several higher-level correlation predictors in the estimation of correlation contributions to reaction energies relative to CCSDT\pQL{}, including Goodson's continued fraction method and a ``new'' method related to \%TAE[(T)] that we refer to as a scaled perturbation estimator. We find that the scaled perturbation estimator based upon CCSD(T\Qf{})/cc-pVDZ is capable of predicting CCSDT\pQL{}/cc-pVDZ contributions to reaction energies with an average error of 0.07 \kcal{} and a RMST of 0.52 \kcal{} when applied to a test-suite of nearly 3000 reactions. This offers a means by which to reliably ballpark how important post-CCSD(T) contributions are to reaction energies while incurring no more than CCSD(T) formal cost and a little mental math.


==> src/discussion.tex <==


